Blocking Self-avoiding Walks Stops Cyber-epidemics: A Scalable GPU-based Approach

Cyber-epidemics, the widespread of fake news or propaganda through social media, can cause devastating economic and political consequences. A common countermeasure against cyber-epidemics is to disable a small subset of suspected social connections or accounts to effectively contain the epidemics. An example is the recent shutdown of 125,000 ISIS-related Twitter accounts. Despite many proposed methods to identify such subset, none are scalable enough to provide high-quality solutions in nowadays billion-size networks. To this end, we investigate the Spread Interdiction problems that seek most effective links (or nodes) for removal under the well-known Linear Threshold model. We propose novel CPU-GPU methods that scale to networks with billions of edges, yet, possess rigorous theoretical guarantee on the solution quality. At the core of our methods is an $O(1)$-space out-of-core algorithm to generate a new type of random walks, called Hitting Self-avoiding Walks (HSAWs). Such a low memory requirement enables handling of big networks and, more importantly, hiding latency via scheduling of millions of threads on GPUs. Comprehensive experiments on real-world networks show that our algorithms provides much higher quality solutions and are several order of magnitude faster than the state-of-the art. Comparing to the (single-core) CPU counterpart, our GPU implementations achieve significant speedup factors up to 177x on a single GPU and 338x on a GPU pair.

==> body/alg.tex <==
\section{Reverse Influence Sampling}
\label{sec:alg}
In this section, we will introduce adaptations of the novel \emph{reverse influence sampling (\RIS{})} technique, originally used in \emph{Influence Maximization (\IM{})} problem \cite{Borgs14,Tang14,Nguyen16}, to the \NRI{} and \ERI{} problems respectively. Then, we propose our first algorithms based on threshold-halting conditions for each problem.

\subsection{Reverse Influence Sampling}
The novel \emph{Reverse Influence Sampling (\RIS{})} technique was first proposed by Borgs et al. \cite{Borgs14} to address the scalability issue of the Influence Maximization (\IM{}), that selects $k$ nodes to maximize their influence, while still maintaining the approximation guarantees. Previously, based on the proof that the influence function (Eq.~\ref{eq:inf}) is \emph{monotone submodular} \cite{Kempe03}, the naive greedy algorithm, that favors to select nodes with highest marginal expected influence, will guarantee a $(1-1/e)$-approximate solution. However, computing marginal expected influence is intractable (\#P-hard) and thus, all of the prior methods resort to simulate the diffusion processes, termed \emph{Forward Sampling}, many times and take the average as a surrogate for the expected influence. Still, the forward sampling substitution is extremely expensive and infeasible for even small-size networks.

Given a probabilistic graph $\mathcal{G}=(\mathcal{V}, \mathcal{E}, w)$, \RIS{} captures the influence landscape of $\G{}$ through generating a set $\R$ of random \textit{Reverse Reachable (RR) sets}. The term `RR set' is also used in \cite{Tang14,Tang15,Nguyen16} and referred to as `hyperedge' in \cite{Borgs14}. Each RR set $R_j$ is a subset of $\mathcal{V}$ and constructed as follows,
\begin{Definition}[Reverse Reachable (RR) set]
	\label{def:rr}
	Given $\mathcal{G}=(\mathcal{V}, \mathcal{E}, w)$, a random RR set $R_j$ is generated from $\mathcal{G}$ by 1) selecting a random node $v \in \mathcal{V}$ 2) generating a sample graph $G$ from $\mathcal{G}$ ($G \sim \G{}$) and 3) returning $R_j$ as the set of nodes that can reach $v$ in $G$.
\end{Definition}
In the above definition, a sample graph $G$ of $\mathcal{G}$ is a deterministic graph where each edge $(u,v) \in \mathcal{E}$ of $\mathcal{G}$ appears in $G$ uniformly with probability $w(u,v)$. Node $v$ in Definition~\ref{def:rr} is called the \emph{source} of $R_j$. A random \RR{} set $R_j$ is actually a random set of nodes that can influence its source. 
%The intuition behind the use of \RR{} set is that if we generate multiple random \RR{} sets, influential nodes will likely appear frequently in the \RR{} sets. Thus a seed set $S$ that \emph{covers} most of the \RR{} sets will likely maximize the influence spread $\I(S)$. Here 
A set $S$ of nodes is said to \emph{cover} an \RR{} set $R_j$, if $S \cap R_j \neq \emptyset$. The following lemma in \cite{Borgs14} reveals how the \RR{} set can be used to compute influence of a set $S$.

\begin{Lemma}[\cite{Borgs14}]
	\label{lem:Borgs}
	Given $\mathcal{G}=(\mathcal{V}, \mathcal{E}, w)$ and a random RR set $R_j$ generated from $\mathcal{G}$. For any node set $S\subset \mathcal{V}$,
	\begin{align}
		\I_{\mathcal{G}}(S) = n \Pr[S \text{ covers } R_j].
	\end{align}
\end{Lemma}

The set $S$ in Lemma~\ref{lem:Borgs} is a fixed set while our suspect set $\V_I$ is stochastic where node $v \in \V_I$ with probability $p(v)$. However, by accounting for all the possible \emph{realizations} $V_I \sim \V_I$, where $v \in V_I$ with $p(v)$ probability, of $\V_I$, we obtain the equivalent lemma for $\V_I$.

\begin{Lemma}
	\label{lem:vi}
	Given $\mathcal{G}=(\mathcal{V}, \mathcal{E}, w)$ and a random RR set $R_j$ generated from $\mathcal{G}$. For each $\mathcal{V}_I\subset \mathcal{V}$ together with $p(v), \forall v \in \V_I$,
	\begin{align}
		\I_{\mathcal{G}}(\V_I,p) = n \Pr[\V_I \text{ covers } R_j].
	\end{align}
\end{Lemma}
\begin{proof}
	Each realization $V_I$ of $\V_I$ is associated with a realization probability,
	\begin{align}
		\Pr[V_I] = \prod_{v \in V_I}p(v)\prod_{v \notin V_I}(1-p(v))
	\end{align}
	Then, the influence of $\V_I$ is computed as follows,
	\begin{align}
		\I(\V_I,p) = \sum_{V_I \sim \V_I}\I(V_I)\Pr[V_I]
	\end{align}
	Since $V_I$ is fixed, apply Lemma~\ref{lem:Borgs} on $\I(V_I)$ on the right-hand side, we obtain,
	\begin{align}
		\I(\V_I,p) & = \sum_{V_I \sim \V_I}n \Pr[V_I \text{ covers } R_j]\Pr[V_I] \\
		& = n \sum_{V_I \sim \V_I} \Pr[V_I \text{ covers } R_j]\Pr[V_I] \\
		& = n \Pr[\V_I \text{ covers } R_j]
	\end{align}
	That completes the proof.
\end{proof}

\subsubsection*{Random \RR{} sets and interdiction problems}

We now connect the idea of random \RR{} sets with our purposes of finding a removal sets of nodes and edges. We say that a set $S \subseteq \mathcal{V}$ \emph{interdicts} the \RR{} set $R_j$ if $S \cap R_j \neq \emptyset$. Similarly, a set $E \subseteq \E{}$ \emph{interdicts} $R_j$ if there is an edge $(u,v) \in E$ and $v, u$ are two consecutive nodes in $R_j$. Combine the concepts of \emph{cover} and \emph{interdict}, we obtain our first lemma for node removal interdiction,
\begin{Lemma}
	\label{lem:rr_node}
	Given $\mathcal{G}=(\mathcal{V}, \mathcal{E}, w)$, a random RR set $R_j$ and a set $\V_I\subset \mathcal{V}$ with $p(v), v\in \V_I$. For any set $S \in \V \backslash \V_I$,
	\begin{align}
		\DN(S,\V_I,p) = n \Pr[(\V_I \text{ covers } R_j) \text{ }\& \text{ } (S \text{ interdicts } R_j)] \nonumber
	\end{align}
\end{Lemma}
\begin{proof}
	Starting from the right-hand side, we have,
	\begin{align}
		\label{eq:eq11}
		&n \Pr[ (S \text{ interdicts } R_j) \text{ }\& \text{ }(\V_I \text{ covers } R_j)] \nonumber \\
		&= n \Pr[(\V_I \text{ covers } R_j)] \Pr[(S \text{ interdicts } R_j) | (\V_I \text{ covers } R_j)] \nonumber \\
		& = \I_{\G{}}(\V_I,p) \Pr[(S \text{ interdicts } R_j) | (\V_I \text{ covers } R_j)]
	\end{align}
	The last equality is obtained from Lemma~\ref{lem:vi}. Note that $\Pr[(S \text{ interdicts } R_j) | (\V_I \text{ covers } R_j)]$ is the probability that $R_j$ is interdicted by $S$ given that $R_j$ is covered by $\V_I$. This probability is exactly equivalent to the fraction of influence blocked by $S$ over the initial influence of $\V_I$. In other words, $\Pr[(S \text{ interdicts } R_j) | (\V_I \text{ covers } R_j)] = \frac{\I_{\G}(\V_I,p) - \I_{\G'}(\V_I,p)}{\I_{\G}(\V_I,p)}$ and replacing to Eq.~\ref{eq:eq11} gives,
	\begin{align}
		\label{eq:eq12}
		n \Pr[ (S & \text{ interdicts } R_j) \text{ }\& \text{ }(\V_I \text{ covers } R_j)] \nonumber \\
		& = \I_{\G{}}(\V_I,p) - \I{\G'{}}(\V_I,p) = \DN(S,\V_I,p)
	\end{align}
	according to Definition~\ref{def:node_remove}. That completes the proof.
\end{proof}
Similarly, we obtain the following lemma for edge removal interdiction problem.

\begin{Lemma}
	\label{lem:rr_edge}
	Given $\mathcal{G}=(\mathcal{V}, \mathcal{E}, w)$, a random RR set $R_j$ and a set $\V_I\subset \mathcal{V}$ with $p(v), v\in \V_I$. For any set $E \in \E$ of edges, we have
	\begin{align}
	\DE(E,\V_I,p) = n \Pr[(\V_I \text{ covers } R_j) \text{ }\& \text{ } (E \text{ interdicts } R_j)] \nonumber
	\end{align}
\end{Lemma}
\newcommand{\twopartdef}[3]
{
	\left\{
	\begin{array}{ll}
		#1 & \mbox{if } #2 \\
		#3 & \mbox{otherwise}
	\end{array}
	\right.
}

Lemmas~\ref{lem:rr_node} and~\ref{lem:rr_edge} state that the expected influence decrease after removing a set of nodes or edges can be analogously computed via \RR{} sets. For each random \RR{} set $R_j$, we define two random variables, $X_j$ and $Y_j$ such that,
\begin{align}
	X_j = \twopartdef {1} {\V_I \text{ covers }R_j \text{ and } S \text{ interdicts }R_j} {0} \nonumber \\
	Y_j = \twopartdef {1} {\V_I \text{ covers }R_j \text{ and } E \text{ interdicts }R_j} {0} \nonumber
\end{align}
From Lemma~\ref{lem:rr_node} and ~\ref{lem:rr_edge}, we obtain,
\begin{align}
	\DN(S,\V_I,p) = n \Pr[X_j = 1]
\end{align}
\vspace{-0.3in}

and
\vspace{-0.1in}
\begin{align}
	\DE(E,\V_I,p) = n \Pr[Y_j = 1]
\end{align}

\subsubsection*{RIS implementation}
Based on Definition~\ref{def:rr}, to generate an \RR{} set, we need a sample graph $G \sim \G{}$ which requires at least $O(n)$ since scanning through all the nodes would take that much time. Instead, we adapt the \RIS{} implementation in \cite{Dinh15} to our scenario of interdiction problems. Specifically, the detailed description is provided in Algorithm~\ref{alg:ris}.

\begin{algorithm}
	\caption{\textsf{\RISLT (\RIS{} sampling for LT model)}}
	\label{alg:ris}
	\KwIn{Graph $\G$, suspect set $\V_I$ and $p(v), \forall v \in \V_I$}
	\KwOut{A random \RR{} set $R_{j}$}
	Pick a node $v$ uniformly at random\\
	$R_j = \emptyset$\\
	\Repeat{$(v \in R_j) \text{ or } v = -1 \text{ or no edge selected }$}{
		Add $v$ to $R_j$\\
		Attempt to select an edge $(u,v)$ using \emph{live-edge} model\\
		\If{edge $(u,v)$ is selected}{
			\If{$u \in \V_I$ \& $rand(0,1) \leq p(u)$}{
				\texttt{// $rand(0,1)$ generates a random number in [0,1] uniformly.}\\
				$u = -1$}
			Set $v = u$}
	}
	Return $R_{j}$\\
\end{algorithm}

The Algorithm~\ref{alg:ris} is based on the \emph{live-edge} version of the LT model described in Section~\ref{sec:model}. The algorithm starts by picking a random source $u$ as the first active node and initializes the \RR{} set to be empty. Subsequently, it follows the live-edge model to repeatedly select the next activated node in the reverse direction (Lines~4-9). This process stops when either the newly activated node creates a loop or determines to be a real threat (Line~7) or no edge has been selected.

The first difference between Alg.~\ref{alg:ris} with the implementation in \cite{Dinh15} is that the set $\V_I$ is stochastic and hence, we have to sample each $v \in \V_I$ with probability $p(v)$ ($rand(0,1)$ at Line~7) to determine whether $v$ is a real threat if $v$ is encountered in the live-edge process. Another distinction of Alg.~\ref{alg:ris} is that it stops whenever a real threat node is encountered since further activations have no effect on the variables $X_j$ and $Y_j$ of that \RR{} set or they do not change the \emph{cover} property of $\V_I$ or \emph{interdict} of $S$ or $E$.

%\subsection{Threshold-halting algorithm}

==> body/analysis.tex <==
\section{Near-optimal Solution Guarantees}
\label{sec:analysis}
